Fine-grained Image Editing by Pixel-wise Guidance Using Diffusion Models

Our goal is to develop fine-grained real-image editing methods suitable for real-world applications. In this paper, we first summarize four requirements for these methods and propose a novel diffusion-based image editing framework with pixel-wise guidance that satisfies these requirements. Specifically, we train pixel-classifiers with a few annotated data and then infer the segmentation map of a target image. Users then manipulate the map to instruct how the image will be edited. We utilize a pre-trained diffusion model to generate edited images aligned with the user's intention with pixel-wise guidance. The effective combination of proposed guidance and other techniques enables highly controllable editing with preserving the outside of the edited area, which results in meeting our requirements. The experimental results demonstrate that our proposal outperforms the GAN-based method for editing quality and speed.

==> subtex_ws/abstract_app.tex <==
% In this study, we tackle the challenges of applying image editing methods to a real-world image editing application.
% In this paper, we first summarize the four requirements for a real-world editing framework, 
% then propose a novel image-editing method based on pixel-wise guidance using diffusion models.
% Specifically, we first train pixel-classifiers with a few annotated data and then estimate the semantic segmentation map of a target image.
% Users then manipulate the map to instruct how the image is to be edited.
% The diffusion model generates an edited image via guidance by pixel-wise classifiers, such that the resultant image aligns with the manipulated map. 
% The effective combination of pixel-wise guidance and other techniques enables reasonable editing in the edited area with preserving the content outside this area and meeting other requirements.
% % The experimental results validate the advantages of the proposed method both quantitatively and qualitatively.
% The experimental results demonstrate that the proposed method outperformed the GAN-based baseline in all metrics and editing speed.


Our goal is to develop fine-grained real-image editing methods suitable for real-world applications.
In this paper, we first summarize four requirements for these methods and propose a novel diffusion-based image editing framework with pixel-wise guidance that satisfies these requirements.
Specifically, we train pixel-classifiers with a few annotated data and then infer the segmentation map of a target image.
Users then manipulate the map to instruct how the image will be edited.
We utilize a pre-trained diffusion model to generate edited images aligned with the user's intention with pixel-wise guidance.
The effective combination of proposed guidance and other techniques enables highly controllable editing with preserving the outside of the edited area, which results in meeting our requirements.
The experimental results demonstrate that our proposal outperforms the GAN-based method for editing quality and speed.
Code is available at \url{https://github.com/sony/pixel-guided-diffusion.git}~\footnote{Code is implemented by NNabla~\cite{narihira2021neural} and pytorch~\cite{paszke2019pytorch}.} 



==> subtex_ws/conclusion.tex <==
In this paper, we proposed a novel fine-grained image editing method using diffusion models in a label-efficient manner.
We achieved precise editing by pixel-wise guidance with pixel classifiers.
Since the guidance is conducted in a pixel-wise manner, the proposed method can jointly achieve both creating reasonable content in the editing region as well as preserving other content in its outside.
The experimental results demonstrate the advantage of our model qualitatively and quantitatively.

==> subtex_ws/introduction.tex <==
%% 問題設定とその難しさを述べる
Recently, generative models have been widely utilized in image-editing methods ~\cite{Croitoru2022DiffusionMI, Xia2022GANIA} thanks to their potential to generate high-quality visual content. 
Several techniques, such as neural photo editing filters, have already been applied to real-world applications by digital artists~\cite{bailey2020tools} and have contributed to expanding their creativity. 
To more effectively reflect the user's intention to the details in edited images, 
we focus on fine-grained image editing. 
In this paper, we refer to fine-grained image editing as an editing process with pixel-level control that does not generates new content but rather makes small and localized changes to the appearance of existing contents in the image, such as manipulating facial parts and animal pose shown in Fig.\ref{fig:overall_results}.
Fine-grained image editing particularly requires two properties: 
(1) visual content in an edited region should be reasonably and locally created according to the user's intention, 
and 
(2) the contents outside the edited region should be precisely preserved. 
Jointly satisfying these two properties leads to higher controllability and better user experience in the editing process.

% Recently, image editing methods based on generative models have become popular~\cite{Croitoru2022DiffusionMI, Xia2022GANIA} thanks to their potential to generate high quality visual content. 
% which is crucial to align with the user's intention. (\textit{e.g.} texts and strokes).
% Then several works, such as neural photo editing filters, 
% have been already applied in real-world applications by digital artists~\cite{bailey2020tools} and have significantly contributed to expanding their creativity.
% To realize the editing which is more faithful to the user's intentions in such applications, fine-grained image editing is essential.
% In this paper, we defined the fine-grained image editing as pixel-wise editing that does not generate new content, but rather makes small localized changes to the appearance of existing content, such manipulation as moving eyes and shortening cat's arm as described in Fig.\ref{fig:overall_results}.
% The users are able to obtain an image that reflects their intent in every details through iterative fine-grained editing as described in Fig.\ref{fig:overall_results}.
% But, we considered that there are two requirements to achieve fine-grained editing, 
% (1) the visual contents in an edited region should be reasonably edited according to the user's intentions, 
% (2) the contents in the outside of the edited region should be precisely preserved.
% This compatibility of them is a significant issue for improvements of fine-grained editing.
In the literature, GANs (Generative Adversarial Networks) ~\cite{goodfellowgenerative} have been intensely adopted for fine-grained image editing ~\cite{Xia2022GANIA,Lee2020MaskGANTD, Park2019SemanticIS,Zhu2020InDomainGI,Ling2021EditGANHS}. 
% These methods generally perform well in a global manner ~\cite{Kwon2022CLIPstylerIS,Patashnik2021StyleCLIPTM, Gal2021StyleGANNADACD, Xia2021TediGANTD, Xu2022TransEditorTD, Shen2020InterpretingTL, Shen2022InterFaceGANIT, Bau2019GANDV, Bau2019SemanticPM,Plumerault2020ControllingGM, Wu2021StyleSpaceAD, Shen2021ClosedFormFO}
% by manipulating latent features corresponding to a target image. 
% For fine-grained editing, 
These methods can precisely reflect fine-grained instruction by users, 
such as manipulated semantic segmentation map ~\cite{Lee2020MaskGANTD, Park2019SemanticIS,Zhu2020InDomainGI,Ling2021EditGANHS}, sketches ~\cite{Chen2020DeepFaceDrawingDG}, into edited images. 
Notably, EditGAN~\cite{Ling2021EditGANHS} is specifically designed to efficiently learn such editing with few annotated segmentation data, which substantially reduces the annotation cost of applying it to a new type of fine-grained image editing.
% But most of them require a large amount of annotated data, then EditGAN~\cite{Ling2021EditGANHS} resolved this drawback using DatasetGAN~\cite{Zhang2021DatasetGANEL}, and achieved fine-grained editing in a label-efficient manner. 
Although these methods successfully provide high-quality visual content in the edited area, it is essentially difficult to strictly preserve other contents in the target image, as shown at the bottom of Fig.\ref{fig:overall_results}, because it requires solving a challenging problem which is to find the latent features corresponding to the edited image while satisfying such constraints. 
% GAN-based methods may cause unintentional change in the visual contents, 
% which are less observed in the training data, outside the edited region (\textit{e.g,} a pacifier in the left case). 
% In the literature, GANs (Generative Adversarial Networks)~\cite{goodfellowgenerative} have been intensely adopted for the image editing. 
% These methods generally perform well on global editing such as ~\cite{Kwon2022CLIPstylerIS,Patashnik2021StyleCLIPTM, Gal2021StyleGANNADACD, Xia2021TediGANTD, Xu2022TransEditorTD, Shen2020InterpretingTL, Shen2022InterFaceGANIT, Bau2019GANDV, Bau2019SemanticPM,Plumerault2020ControllingGM, Wu2021StyleSpaceAD, Shen2021ClosedFormFO} by manipulating latent features corresponding to a target image. As for fine-grained and localized editing, several studies extend these methods to precisely reflect fine-grained instruction by users, 
% such as manipulation of a semantic segmentation map, an object mask, or sketches~\cite{Lee2020MaskGANTD, Park2019SemanticIS,Zhu2020InDomainGI,Chen2020DeepFaceDrawingDG,Ling2021EditGANHS}, into edited images. 
% Although these methods can provide high-quality visual contents in the edited area, 
% it is essentially difficult to strictly preserve other contents in the target image. This is because it is still difficult to find the appropriate latent variables corresponding to the real images, despite there are many GAN inversion techniques~\cite{Abdal2019Image2StyleGANHT,Abdal2020Image2StyleGANHT,Alaluf2021ReStyleAR,Richardson2021EncodingIS,Tov2021DesigningAE,Zhu2020InDomainGI, Alaluf2022HyperStyleSI}. 


% To solve these issues, GAN(Generative Adversarial Network)~\cite{goodfellowgenerative}-based image editing methods, such as user-provided text-based editing methods~\cite{Kwon2022CLIPstylerIS,Patashnik2021StyleCLIPTM, Gal2021StyleGANNADACD, Xia2021TediGANTD} and latent manipulation methods~\cite{Xu2022TransEditorTD, Shen2020InterpretingTL, Shen2022InterFaceGANIT, Bau2019GANDV, Bau2019SemanticPM,Plumerault2020ControllingGM, Wu2021StyleSpaceAD, Shen2021ClosedFormFO}, have been studied well.
% These methods achieved global editing like style transfer and attribute transformation.
% For fine-grained and localized editing, there are several methods using segmentation maps and masks and skethces~\cite{Lee2020MaskGANTD, Park2019SemanticIS,Zhu2020InDomainGI,Chen2020DeepFaceDrawingDG}.
% However, in situations such as real image editing, all these GAN-based methods should invert those images to their learned latent spaces.
% Although, there are many inversion techniques~\cite{Abdal2019Image2StyleGANHT,Abdal2020Image2StyleGANHT,Alaluf2021ReStyleAR,Richardson2021EncodingIS,Tov2021DesigningAE,Zhu2020InDomainGI, Alaluf2022HyperStyleSI}, 
% it has a strict trade-off between editability and reconstruction performance of inverted images.
% As a result, gan-based editing methods have a difficulty on editing only desired regions with preserving the features of out these regions.


% For real image editing, denoising diffusion probabilistic model(DDPM) ~\cite{Ho2020DenoisingDP,SohlDickstein2015DeepUL,Nichol2021ImprovedDD,Dhariwal2021DiffusionMB} and score-based generative models~\cite{Song2019GenerativeMB, Song2021ScoreBasedGM} are suitable.
% Because its outperformed image synthesis quality~\cite{Dhariwal2021DiffusionMB} against existing generative models~\cite{brock2018large, kingma2013auto, van2016pixel, menick2018generating, rezende2015variational} and accurate reconstruction performance thanks to DDIM~\cite{Song2021DenoisingDI}.
% Therefore, a lot of real image editing methods with diffusion models have been emerged.
% For fine-grained editing, diffusion-based methods are divided into two categories.
% One line of research are training conditional diffusion models~\cite{Nichol2022GLIDETP, Saharia2022PaletteID}.
% It enables localized editing by training diffusion models with such conditional input, but high training cost is drawback.
% However, unconditional model based methods~\cite{Choi2021ILVRCM,Meng2021SDEditIS,avrahami2022blended,Avrahami2022BlendedLD}, it can use the pre-trained diffusion models, achieve editing with low training cost.
% These methods achieved localized editing useing texts and strokes.
% But it is difficult for precise editing using only text and some stroke-based methods have a strict trade-off, which is difficult for non-specialist to control, between realism and faithfullness.


% Then, in the recent works of image synthesis, denoising diffusion probabilistic model (DDPM)~\cite{Ho2020DenoisingDP,SohlDickstein2015DeepUL,Nichol2021ImprovedDD,Dhariwal2021DiffusionMB} and score-based generative models~\cite{Song2019GenerativeMB, Song2021ScoreBasedGM} have been attracted much attention.
% These models are categorized to a probabilistic generative model which can generate diverse images.
% The latest works~\cite{Dhariwal2021DiffusionMB} shows a outperforming image synthesis quality against existing generative models~\cite{brock2018large, kingma2013auto, van2016pixel, menick2018generating, rezende2015variational}.
% From a point view of real image editing, 
% we can obtain accurate reconstruction images using a denoising diffusion implicit models(DDIM)~\cite{Song2021DenoisingDI}.
% It resolved the aforementioned problems in GANs' inversion performance. 
% Therefore, a lot of real image editing methods using diffusion models have been emerging.
% Some approaches are text-based editing~\cite{avrahami2022blended, Avrahami2022BlendedLD, Kim2022DiffusionCLIPTD}.
% These methods can edit real images by user-provided text prompts thanks to the ability of Contrastive Language-Image Pretraining (CLIP)~\cite{Radford2021LearningTV}.
% And DreamBooth~\cite{Ruiz2022DreamBoothFT} can appear personalized objects on other contexts images according to text prompts.
% However, text-based methods could not edit images to reflect the user's intent down to the small details of the images.
% Another methods are conditioning on generation~\cite{Choi2021ILVRCM, Preechakul2022DiffusionAT} using reference images and interpolation techniques and so on.
% SDEdit~\cite{Meng2021SDEditIS} can edit images using storke and skethces, then realize editing which is reflected human intuitive intent. 
% But it has a trade-off between realism and faithfullness. 
% This is difficult for non-specialists to control this trade-off.

% To address this issue, we use diffusion models instead of GANs and introduced a novel image editing method based on user-provided pixel-wise manipulation of semantic segmentation map.
% Specifically, we first train pixel-classifiers~\cite{Baranchuk2022LabelEfficientSS} with few annotated data and then apply them to a target image to estimate its semantic segmentation map.
% Users manipulate this map to instruct how the target image is to be edited, 
% and the diffusion model generates an edited image via pixel-wise guidance.
To address the above-mentioned issue, we adopt diffusion models instead of GANs, then propose a novel fine-grained image editing method based on pixel-wise guidance with a few annotated data. 
For guidance, we first train pixel classifiers that to estimate the semantics of a target pixel. 
The classifiers are then used to guide the generation process by the diffusion model so that the generated image aligns with an edited semantic segmentation map. 
Since this guidance is conducted in a pixel-wise manner, 
our method can precisely preserve content outside an edited area while creating reasonable content in the edited area. 
Experimental results validate the advantage of our method compared with GAN-based methods both quantitatively and qualitatively.


In summary, our contributions are three-fold: 
\begin{itemize}
\setlength{\parskip}{0cm}
\setlength{\itemsep}{0cm}
\item We propose a novel image editing method based on pixel-wise guidance using diffusion models in a label-efficient manner.
\item We reveal that the optimal setting of both start denoising step $t_0$ and guidance scale $s$ depends on the size of the edited region. This finding is helpful in determining the parameter setting for unseen test data.
\item We reveal that there are disentangled latent vectors on the latent space of the pre-trained ADM. It is helpful to control the intensity of editing.
\item Our guidance technique is more computationally efficient than the conventional guidance based on full-size segmentation models. It contributes to fast editing.
% \item Our method achieved computationally more efficient guidance than using full-size segmentation models for guidance. It is helpful for fast editing.

\end{itemize}






